Bayesian Level Set Clustering

Classically, Bayesian clustering interprets each component of a mixture model as a cluster. The inferred clustering posterior is highly sensitive to any inaccuracies in the kernel within each component. As this kernel is made more flexible, problems arise in identifying the underlying clusters in the data. To address this pitfall, this article proposes a fundamentally different approach to Bayesian clustering that decouples the problems of clustering and flexible modeling of the data density $f$. Starting with an arbitrary Bayesian model for $f$ and a loss function for defining clusters based on $f$, we develop a Bayesian decision-theoretic framework for density-based clustering. Within this framework, we develop a Bayesian level set clustering method to cluster data into connected components of a level set of $f$. We provide theoretical support, including clustering consistency, and highlight performance in a variety of simulated examples. An application to astronomical data illustrates improvements over the popular DBSCAN algorithm in terms of accuracy, insensitivity to tuning parameters, and providing uncertainty quantification.

==> thm1-assumptions.tex <==


We now discuss the assumptions underlying \Cref{thm:consistency}. Starting from the assumptions the proof of \Cref{thm:consistency}, provided in \Cref{ss:proof-of-consistency}, is a simple application of the triangle inequality. The proof essentially captures the intuition that as long as the posterior distribution of $f$ is concentrated around $f_0$ (\Cref{ass:sup-norm-concentration}) in terms of a metric $\rho$ that can guarantee that the clustering $\psi(f)$ and $\psi(f_0)$ are close (\Cref{ass:continuity-at-f0}) in terms of $D$, then the Bayes optimal estimated clustering will also be close to $\psi(f_0)$ 

\begin{assumption}
	Suppose that $D:  \ClustSpace[\cX_n] \times  \ClustSpace[\cX_n] \to [0,1]$ is a metric. 
	\label{ass:dist-bounded}
\end{assumption}

We assume that the loss $D$ is a metric bounded above by one. While we can enforce boundedness by suitably re-scaling $D$ or replacing it by $\max(D,1)$, the metric properties of $D$, particularly non-negativity, symmetry, and triangle inequality, are crucially used in the proof of \Cref{thm:consistency}.

Next, we assume that the Bayesian model $M$ for the unknown density $f$ is such that its posterior distribution $P_M(\cdot|\cX_n)$, under samples $\cX_n = \{ x_1, \ldots, x_n \}$ drawn independently from $f_0$,  
 contracts at rate $\epsilon_n$ to $f_0$ in some metric $\rho$ on the space of densities $\Den$. %

\begin{assumption}[Posterior contraction] If $\cX_n = \{ x_1, \ldots, x_n \}$ are drawn independently from $f_0$, then there is a metric $\rho$ on $\Den$ and non-random sequence $\{\epsilon_n\}_{n \geq 1} \subseteq \R_{+}$ such that 
	$$
	\tau_{1}(\cX_n) \doteq P_M\left(f : \rho(f,f_0) \geq \epsilon_n K_n \big| \cX_n\right) \pconv 0
	$$
	as $n \to \infty$, for every sequence $\{K_n\}_{n \in \nat} \subseteq \R$ such that $\lim_{n \to \infty} K_n = \infty$. 
	\label{ass:sup-norm-concentration}
\end{assumption}


\begin{assumption} Suppose that $\tau_{2}(\cX_n) \doteq \sup_{f \in \Den : \rho(f,f_0) \leq K_n \epsilon_n} D\{\psitilde(f), \psi(f_0)\} \pconv 0$ as $n \to \infty$ for some sequence $K_n \to \infty$. Here $\rho$ and $\epsilon_n$ are as given in \Cref{ass:sup-norm-concentration}.
	\label{ass:continuity-at-f0}
\end{assumption}	


Note that \Cref{ass:continuity-at-f0,ass:sup-norm-concentration} are related to each other in that we need a common sequence $\{(\epsilon_n, K_n)\}_{n \geq 1}$ and the same metric $\rho$ on $\Den$ such that both \Cref{ass:continuity-at-f0,ass:sup-norm-concentration} hold. 
While \Cref{ass:sup-norm-concentration} is similar to a standard posterior contraction result, \Cref{ass:continuity-at-f0} requires that the distance between the surrogate clustering $\psitilde(f)$ and the true clustering $\psi(f_0)$ will be small in the metric $D$ when $f$ is suitably close to $f_0$ in the metric $\rho$. Intuitively, this requires that (a) $\psitilde$ is an accurate surrogate for $\psi$, and (b) $\psi$ is continuous at $f_0$ with respect to the metric $\rho$. 


While standard posterior contraction results (??) establish the convergence in \Cref{ass:sup-norm-concentration} when $\rho$ is the Hellinger metric, convergence guarantees in stronger metrics will typically be required that can ensure continuity of clustering functional $\psi: \Den \to \ClustSpace[\cX_n]$. For instance, to establish consistency for level-set clustering in \Cref{ss:prove-level-set-clustering} we will take $\rho(f,g) = \|f-g\|_\infty \doteq \sup_{x \in \cX} |f(x) - g(x)|$ to be the $L_\infty$ norm. Similarly, capuring both the posterior contraction of the density $f$ along with its derivatives will seemingly be required when $\psi$ represent modal clustering \cite[see][]{shen2017posterior}. Thus, esablishing posterior rates of convergence with stronger metrics $\rho$ than the Hellinger distance is an active area of research \citep{gine2011rates,  
castillo2014bayesian,castillo2017polya,naulet2022adaptive,shen2017posterior,li2021posterior}, which can ensure consistency of Bayesian density-based clustering procedures shown here \Cref{thm:consistency}. 



Establishing posterior contraction in the $L_\infty$ metric, as required by \Cref{ass:sup-norm-concentration}, is an active area of research.
For univariate density estimation on $\cX=[0,1]$, such contraction rates have been established for 
kernel mixture models, random histogram priors, P\'olya trees, Gaussian process and wavelet series priors on the log density
\citep{gine2011rates,  
castillo2014bayesian,castillo2017polya,naulet2022adaptive}. 
For multivariate density estimation on $\cX = [0,1]^d$, %
refer to 
\cite{li2021posterior} and references therein. %





==> verify-BALLET-assumptions.tex <==


As mentioned above, verifying \Cref{ass:sup-norm-concentration}, which describes posterior contraction for the Bayesian density model $M$ in the $L_\infty$ norm, constitutes an active area of research in Bayesian nonparametrics. We now verify \Cref{ass:continuity-at-f0,ass:dist-bounded} for the setup of \texttt{BALLET} Estimators. 

The following theorem proved in \Cref{ss:metric-properties} shows that \Cref{ass:dist-bounded} is satisfied for suitable choices of constants in our Inactive/Active Binder's loss \eqref{eq:ia-binder-loss}.

\begin{theorem}  Suppose $0 < a = b \leq 1$, $m = m_{ia} = m_{ai} \leq 1$, and $a \leq 2m$. Then $D = \binom{n}{2}^{-1} \Lia$ is a metric on $\ClustSpace[\cX_n]$ that is bounded above by 1.
	\label{lem:IABender-is-a-metric}
\end{theorem}

We now verify  \Cref{ass:continuity-at-f0} in this setup for some mild conditions on the density $f_0$  stated in \Cref{ss:prove-level-set-clustering}. We roughly require that $f_0: \R^d \to [0,\infty)$ is continuous and vanishing in the tails (\Cref{ass:uniform-continuity}), is not flat around the level $\lambda$ (\Cref{ass:mass-decay}), and has a level-$\lambda$ clustering that is stable with respect to small perturbations in $\lambda$ (\Cref{ass:robust-cluster}). %
The condition $\delta_n \geq \rnld$ in the following theorem is used to ensure that the tube-based estimator $T_{\delta_n}(A_{f, \lambda})$ from \Cref{ss:surrogate-clustering-function} is a consistent estimator for $S_\lambda$. 




\begin{theorem} Suppose $\cX = \R^d$ and the density $f_0$ satisfies \Cref{ass:uniform-continuity,ass:mass-decay,ass:robust-cluster} in \Cref{ss:prove-level-set-clustering} and is 
$\alpha$-H\"older smooth for some $\alpha \in (0,1]$. Let $\cX_n = \{x_1, \ldots, x_n\}$ be drawn independently from $f_0$, $D$ be the re-scaled loss from \Cref{lem:IABender-is-a-metric}, and $\{\delta_n\}_{n \geq 1}$ be any sequence converging to zero such that $\delta_n \geq 2\rnld$, where $\rnld = \rnldval$, $\lambda > 0$ is the chosen level, $\Gamma$ is  the gamma function, and $C_1 \geq 1$ is a universal constant.  Then for any sequence $\{(K_n, \epsilon_n)\}_{n \geq 1} \subseteq \R^2_+$ such that $K_n \epsilon_n \to 0$, \Cref{ass:continuity-at-f0} is satisfied for the BALLET estimator with $\psitilde = \psiclust[\delta_n]$ and $\psi  = \psi_\lambda$. In particular,
	$$
	\tau_2(\cX_n) = \sup_{f: \|f-f_0\|_\infty \leq K_n \epsilon_n } D\{\psiclust[\delta_n](f), \psi_\lambda(f_0)\} \leq C_0 \bigg\{\max(K_n \epsilon_n, \delta_n^{\alpha}) + \sqrt{\frac{\ln n}{n}} \bigg\} 
	$$
	with probability at least $1-\frac{2}{n}$ when $n \geq n_0$. Here $C_0, n_0 > 0$ are finite constants that may depend on $f_0$ and the sequences $\{(\delta_n, K_n, \epsilon_n)\}_{n \geq 1}$ but are independent of $n$ and data $\cX_n$.
	\label{lem:finite-sample-bound-for-assumption2}
\end{theorem}






Thus an application of \Cref{thm:consistency} shows
\begin{equation}
	\binom{n}{2}^{-1}\Lia\{\BALLET[\delta_n], \psi_\lambda(f_0)\} \pconv 0  \qquad \text{as } n \to \infty,
	\label{eq:re-scaled-binder-consistency}
\end{equation}
whenever $\cX_n = \{x_1, \ldots, x_n\}$ are independent from $f_0$ and loss $\Lia$ satisfies conditions of \Cref{lem:IABender-is-a-metric}. 

From the sum-based representation of $\Lia$ in \cref{eq:sum-representation}, we note that the convergence in \Cref{eq:re-scaled-binder-consistency} implies that only a vanishingly small fraction of pairs of points from $\cX_n$ can be clustered differently between $\BALLET[\delta_n]$ and $\psi_\lambda(f_0)$ as $n \to \infty$.

